Learning Portrait Style Representations

Style analysis of artwork in computer vision predominantly focuses on achieving results in target image generation through optimizing understanding of low level style characteristics such as brush strokes. However, fundamentally different techniques are required to computationally understand and control qualities of art which incorporate higher level style characteristics. We study style representations learned by neural network architectures incorporating these higher level characteristics. We find variation in learned style features from incorporating triplets annotated by art historians as supervision for style similarity. Networks leveraging statistical priors or pretrained on photo collections such as ImageNet can also derive useful visual representations of artwork. We align the impact of these expert human knowledge, statistical, and photo realism priors on style representations with art historical research and use these representations to perform zero-shot classification of artists. To facilitate this work, we also present the first large-scale dataset of portraits prepared for computational analysis.

==> tex/metric_learning.tex <==
\section{Deep Metric Learning}
The Triplet Loss was first introduced in \cite{hoffer2015deep} and has since been used such as in \cite{Schroff2015} for deep metric learning. Additionally, Variational Autoencoders (VAE), first introduced in \cite{Kingma2014} have enjoyed recent success in the Deep Learning, and specifically explainable AI community due to their ability to learn a semantic, latent subspace of a dataset. Due to the VAE's ability to learn a rich subspace and a triplet loss for deep metric learning, we combine both approaches using professionally labeled triplets to learn a latent style representation of our curated Portrait Dataset. \\

\noindent Traditionally, the loss function for a VAE is defined as follows:
\begin{equation}
    \mathcal{L}_{\text{VAE}} = \lambda_1 \mathcal{L}_{KL} + \lambda_2 \mathcal{L}_{RECON} = \lambda_1 D_{KL}\left(p_{\theta}(z | x)\Vert\mathcal{N}(0,1)\right) + \lambda_2 \Vert I-\widehat{I} \Vert^2_2
\end{equation}
$\mathcal{L}_1$ is the KL Divergence of the latent distribution $p_{\theta}(z | x)$ with respect to the assumed prior unit standard Gaussian distribution $\mathcal{N}(0, 1)$ of each feature $z_i \in z$. $L_2$ is also known as the ``Reconstruction Loss", which enforces that the latent representation $z$ can also be decoded to generate $\widehat{I}$, which closely matches the input image $I$. \\\\
In our approach, we introduce two additional losses to increase the quality of reconstructions $\widehat{I}$ as well as ensure that the learned subspace captures attributes of style. The first added loss is a super-resolution perceptual loss, first introduced in \cite{Johnson2016Perceptual}, which helps circumvent the issues with just using a mean-squared error as discussed in \cite{Mathieu2016}. The second added loss is a triplet loss, which is defined similarly to that of FaceNet in \cite{Schroff2015}. Formally, we define our triplet loss to be:
\begin{align}
\mathcal{L}_{TRIPLET} &= \frac{\lambda_{4}}{\max(N_{+}, 1)}\sum_{i}^N \left[\left\|\mu_a-\mu_p\right\|_{2}^{2}-\left\|\mu_a- \mu_n\right\|_{2}^{2}+\alpha \right]_{+}
\end{align}
Where:
\begin{align}
N_{+} &= \sum_{i}^N \mathbbm{1} (\left\|\mu_a-\mu_p\right\|_{2}^{2}-\left\|\mu_a- \mu_n\right\|_{2}^{2}+\alpha > 0)
\end{align}
$\mu_{a}, \mu_{p}, \mu_{n}$ are the means for the latent representations of the anchor, positive, and negative images in the triplet respectively.\\\\
Typically when employing a triplet loss, triplet mining is done to only extract the hardest of the polynomial number of possible triplets, however, this requires that the label can be automatically determined for any arbitrary triplet. In our approach, triplets require professional labelling, therefore we cannot employ traditional triplet mining techniques as
described in \cite{DBLP:journals/corr/HermansBL17,Schroff2015}. Instead we avoid training on triplets that trivially satisfy the triplet constraint by normalizing the loss by only the number of triplets, $N_{+}$, that do not already satisfy the triplet constraint. We combine all of the aforementioned losses to get the final training objective:
\begin{equation}
    \mathcal{L}_{\text{VAE}} = \lambda_1 \mathcal{L}_{KL} + \lambda_2 \mathcal{L}_{RECON} + \lambda_3 \mathcal{L}_{TRIPLET} + \lambda_4 \mathcal{L}_{PERCEP}
\end{equation}
Where $\mathcal{L}_{PERCEP}$ is the super-resolution perceptual loss. The full model architecture can be viewed in Figure \ref{fig:vae} \\\\
\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.13]{eccv2020/figures/architecture.png}
    \caption{VAE Model Architecture}
    \label{fig:vae}
\end{figure*}
We show through this approach the ability of the model to not only reconstruct the input data but also be able to generate novel artwork, as demonstrated in Figure \ref{fig:reconstructions}. Though novel style-conditioned portrait synthesis confirms some of the intended behavior of our trained model, our primary purpose of this work is to learn a meaningful style distribution of art portraiture. Thus, our primary experiments focus on the analysis of the clustering in this learned style space as well as analyzing the difference in feature activations from the learned models.

% If our faces don't have features after tuning latent space size, length of training, depth of network, kl v rec loss weights:
% 1. GAN-VAE
% 2. Perceptual loss in VAE

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.5]{eccv2020/figures/annotated_recons.png}
    \caption{Reconstructions from our VAE of portraits in our test set. The first row is the linear interpolation between the source and target test set images with factor $t$. The second row is the reconstruction $q_{\phi}(x | z)$ where the latent $z$ is linearly interpolated from the source and target latent representations.}
    \label{fig:reconstructions}
\end{figure}

%TODO include data about anonymous in supplementary material

\subsection{Latent Space Analysis}
\subsubsection{Style Embedding Clustering}
To analyze the embeddings produced for each model, we use PCA and TSNE to project the embeddings into a 2 dimensional space. We then project all of the embeddings in the test set to this 2D space and only visualize the points from the 5 most represented artists.

\newpage
\begin{figure}
\centering
\begin{subfigure}{.9\linewidth}
    \centering
    \includegraphics[scale=0.2]{eccv2020/figures/latent_plots/NoTriplet.png}
    \caption{2D TSNE Projection of test set embeddings from VAE model trained \textbf{without} triplet loss}
    \label{fig:notriplet}
\end{subfigure}
\begin{subfigure}{.9\linewidth}
    \centering
    \includegraphics[scale=0.2]{eccv2020/figures/latent_plots/Triplet.png}
    \caption{2D TSNE Projection of test set embeddings from VAE model trained \textbf{with} triplet loss}
    \label{fig:notriplet}
\end{subfigure}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{.9\linewidth}
    \centering
    \includegraphics[scale=0.2]{eccv2020/figures/latent_plots/VGG.png}
    \caption{2D TSNE Projection of test set embeddings from pretrained VGG-16 model}
    \label{fig:vgg}
\end{subfigure}
\begin{subfigure}{.9\linewidth}
    \centering
    % \includegraphics[scale=0.2]{eccv2020/figures/latent_plots/VGG.png}
    \caption{2D TSNE Projection of test set embeddings from using VGG-16 as the VAE encoder}
    \label{fig:vgg}
\end{subfigure}
\end{figure}


% We first show the success of our method to perform latent partitioning by artist and time-period by generating t-sne plots of each of these latent components, $z_a$ and $z_t$, in Figure \ref{fig:latents}. With this analysis, we show that these separate latent components are clustered by artist and time period in each feature space. These clusters visualize the learned correlation of distinct style features with artist and time period data within different portions of the latent space.

% We observe from Figure \ref{fig:artists_dist} that we have many images for which there is only one artist. However, Figure \ref{fig:20art} shows that the representation of the top 20 artists in our dataset is much higher. Thus, in our t-sne visualization, we only color features associated with the top 20 artists so that we can highlight the artist style representations which have enough data to be associated with significantly sized latent clusters. All other points are left grey. Figure \ref{fig:latents}.a. shows this feature space clustering.

% %TODO add time period data distribution visualization

% \begin{figure*}[h]
%     \centering
%     %\includegraphics[scale=0.6]{latex/figures/figure4.jpg}
%     \caption{T-sne of artist and time period latent space.}
%     \label{fig:latents}
% \end{figure*}

% % TODO we could also go into some detail of what portraits are close in time versus artist space if there is time

% Our data does not include distinct labels for time periods in the same manner as the artist information. Since the portraits in our data are associated with time ranges instead of individual dates, we have cases in which one portrait may have a time range nested within the time range of a different portrait. However, given the variation of this overlap, we are still able to gather understanding of distinct blocks of time associated with distinct contributions of style. We take the full range of the time period distribution represented in our dataset and separate this range into 5 blocks equal in time duration. The clustering of the style representations associated with each of these time blocks is shown in Figure \ref{fig:latents}.b. %TODO tune the number of time blocks

% We note that a well-defined association between the image time period labels and our time blocking approach for identifying feature space clusters needed to be constructed for this analysis. If a block of time is entirely contained within the range associated with an image, then points in the feature space are given a color associated with that block of time. However, if an image time range encompasses multiple blocks, then the feature space points are colored associated with a gradient between the colors attributed to individual blocks. The gradient color is computed using a fractional contribution of each base color associated with the degree of overlap between the boxes.


% % This differs slightly from \cite{Schroff2015} in that we normalize the triplet loss by $N_{+}$, which is the number of non-trivial triplets in the mini-batch. Typically when employing a triplet loss, triplet mining is done to 
% % This is done because unlike \cite{Schroff2015} the triplet labels are professionally annotated. Thus, we do not have a polynomial number of triplets to construct and thus to help convergence we only normalize the samples which 



% % Variational Autoencoders are known to learn semantic latent representations and as such, our approach leverages t

% % Derive losses from the probabilistic formulation of the VAE as a graphical model

% % Present the theory of disentanglement - deriving z1 and z2 separately from z

% \begin{figure*}[t]
%     \centering
%     \includegraphics[scale=0.13]{eccv2020/figures/architecture.png}
%     \caption{VAE Model Architecture}
%     \label{fig:vae}
% \end{figure*}

% Add probabilistic model intro here. We use VAEs because they are good generative models. This is their loss function.



% The VAE in our architecture is visualized in Figure \ref{fig:vae}.

% To partition the latent space $z$ of our VAE, we fix a dimension for each latent subspace which corresponds to each artistic property we disentangle in the feature space. Then, we use that latent representation to predict associated labels for the image. We combine the losses from these predicted characteristics in a total loss with the VAE losses so that the latent space is partitioned through the training process. We use this procedure for disentanglement to separate latent style features associated the artist, the time period, and other differences derived from professional identified similarity. This disentangling procedure is visualized in Figure \ref{fig:disentangle}.

% \begin{figure}[h]
%     \centering
%     %\includegraphics[scale=0.7]{latex/figures/figure2.jpg}
%     \caption{Architecture for disentangling the latent representations of style.}
%     \label{fig:disentangle}
% \end{figure}

% To enforce separation of artist-defined style in the latent space, latent features in a subset of $z$ are used to predict the artist attribution for the image. The loss associate with this prediction is defined as

% \begin{equation}
%     L_3 = \Vert x - \widehat{x} \Vert_1
% \end{equation}

% where $x$ is the true artist and $\widehat{x}$ is the predicted artist.

% %TODO explain handling for uncertain author attribution

% We use the latent style representation we associate with time period-defined style to predict a time-period distribution. This distribution is assumed to be Gaussian centered in the midpoint of the given range. Thus, the loss used to enforce separation is given by the KL-divergence as specified below.

% \begin{equation}
%     L_4 = D_{KL}\left(y \Vert \widehat{y} \right)
% \end{equation}

% We denote the true time period distribution as $y$ and the predicted distribution as $\widehat{y}$. Note that some of our metadata includes a single year instead of a distribution. For consistency in our analysis, we 

% We define our triplet loss to force similarity in the latent space. \cite{tripletLoss}

% \begin{equation}
%     L_5 = \max \left( D_{KL}(z_o^a \Vert z_o^p) - D_{KL}(z_o^a \Vert z_o^n) + \alpha , 0\right)
% \end{equation}

% With these loss contributions, we define our total loss as 
% \begin{equation}
%     L_{\text{total}} = \sum_{i=1}^5 \lambda_i L_i
% \end{equation}

==> tex/novel_images.tex <==

\subsection{Novel Artwork Generation}

% % Reason for not baseline artgan: In addition, the GAN generator is only compatible with one style, so a series of GANs must be trained to provide users with choices to transfer more than one kind of style.

% We now demonstrate the capability of our method to generate new artwork in target style combinations isolated by our network. Through our latent space analysis, we discovered the decision boundaries associated with specific time periods and artists. Thus, we can isolate the response in our network for an arbitrary artist or time period such that the probability of artwork decoded from that latent space to be associated with those fixed attributes is highest.

% In our image generation experiments, we manually fix the network response for a set artist and time period at a point of strongest association while varying the other latent style component captured by our triplet loss. We then use these latent space constructions to decode a novel image. Using this procedure, we generated 50 novel images for each of 10 distinct artist-time period pairs. We then created a triplet for each novel image which included an anchor image with a given artist-time period pair, an image with the same artist-time period pair, and an image with a different artist-time period pair. We had 3 professional art historians choose the image in each triplet which they anticipated came from the same artist and time period as the anchor image. 

% We report a human agreement score for the professionally assigned labels by computing an agreement percentage for all the triplets. Individual agreement scores are 1 for the triplets for which all 3 artists agree and 0 for the triplets for which they do not agree. We also track a human-machine agreement score as the percent of generated images for which both the majority art historian opinion and our network identify as having the same artist-time period style. These results are shown in Table \ref{tab:machine_test}. Having a close agreement score indicates that our network is interpreting style in a manner comparable to professional human interpretation. %TODO add in a comment on actual observed results
% We also observe a direct relationship between the human agreement score and human-machine agreement score shown in Figure \ref{fig:agree} demonstrating the similarity in human and machine style analysis. 

% Select visualizations from our reconstructions are shown in Figure \ref{fig:reconstructions}. We reiterate that the goal of our work is to develop human-like interpretations and understanding of style as opposed to generating the most high fidelity target paintings. We acknowledge that some of our artwork seems to have less sharp reconstructions of facial features than intended, but we note that the professional analysis of this artwork is comparable to an art historian inspecting artwork which may be damaged. Our human triplet labels were given in the same manner as though they were inspecting the image of a previously unseen work of art without knowledge of its origins. 

% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c|c}
%          & Human Agreement & Human-Machine \\
%          & & Agreement \\
%          \hline \\
%         Artist 1 & \% & \% \\
%          Time Period 1 & & \\
%          & & \\
%         Artist 2 & \% & \% \\
%         Time Period 2 & & \\
%          & & \\
%         Artist 3 & \% & \% \\
%         Time Period 3 & & \\
%          & & \\
%         Artist 4 & \% & \% \\
%         Time Period 4 & & \\
%          & & \\
%         Artist 5 & \% & \% \\
%         Time Period 5 & & \\
%          & & \\
%         Artist 6 & \% & \% \\
%         Time Period 6 & & \\
%          & & \\
%         Artist 7 & \% & \% \\
%         Time Period 7 & & \\
%          & & \\
%         Artist 8 & \% & \% \\
%         Time Period 8 & & \\
%          & & \\
%         Artist 9 & \% & \% \\
%         Time Period 9 & & \\
%          & & \\
%         Artist 10 & \% & \% \\
%         Time Period 10 & &
%     \end{tabular}
%     \caption{Percentage match in artist-time period label assignments between our network and a professional art historian over 50 generated images for each label pair.}
%     \label{tab:machine_test}
% \end{table}

% \begin{figure}[t]
%     \centering
%     %\includegraphics[scale=0.2]{latex/figures/figure5.jpg}
%     \caption{Relationship between human agreement and human-machine agreement scores.}
%     \label{fig:agree}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     %\includegraphics[scale=0.8]{latex/figures/figure1.jpeg}
%     \caption{Novel artwork generation samples for different artist-time period pairs used in the human experiments.}
%     \label{fig:art_gen}
% \end{figure}
